Efficient Sensorimotor Learning for Open-world Robot Manipulation

This dissertation considers Open-world Robot Manipulation, a manipulation problem where a robot must generalize or quickly adapt to new objects, scenes, or tasks for which it has not been pre-programmed or pre-trained. This dissertation tackles the problem using a methodology of efficient sensorimotor learning. The key to enabling efficient sensorimotor learning lies in leveraging regular patterns that exist in limited amounts of demonstration data. These patterns, referred to as ``regularity,'' enable the data-efficient learning of generalizable manipulation skills. This dissertation offers a new perspective on formulating manipulation problems through the lens of regularity. Building upon this notion, we introduce three major contributions. First, we introduce methods that endow robots with object-centric priors, allowing them to learn generalizable, closed-loop sensorimotor policies from a small number of teleoperation demonstrations. Second, we introduce methods that constitute robots' spatial understanding, unlocking their ability to imitate manipulation skills from in-the-wild video observations. Last but not least, we introduce methods that enable robots to identify reusable skills from their past experiences, resulting in systems that can continually imitate multiple tasks in a sequential manner. Altogether, the contributions of this dissertation help lay the groundwork for building general-purpose personal robots that can quickly adapt to new situations or tasks with low-cost data collection and interact easily with humans. By enabling robots to learn and generalize from limited data, this dissertation takes a step toward realizing the vision of intelligent robotic assistants that can be seamlessly integrated into everyday scenarios.

==> structural/body.tex <==
% This is the body of your document. You may copy-paste it into your main document
% (dissertation.tex, masterreport.tex, masterthesis.tex, treatise.tex), or edit it here.


\copyrightpage  % Produces the copyright page. Optional.

\commcertpage   % Produces the Committee Certification
			%   of Approved Version page (doctoral)
			%   or Signature page (masters).
			%		20 Mar 2002	cwm
                % Required.

\titlepage      % Produces the title page. Required.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Dedication and/or epigraph are optional, but must occur here.      %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{dedication}		% Optional
To all future Longhorn graduate students.
\end{dedication}

\begin{epigraph}		% Optional
\begin{center}
    \textit{What starts here changes the world.}
    \\\hspace{4em}---University of Texas at Austin
\end{center}
\end{epigraph}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Acknowledgements and/or preface are optional, but must occur here. %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{acknowledgments}		% Optional
Thanks to the previous authors of this template, and to the Graduate School for providing it.
\end{acknowledgments}

\begin{preface}		% Optional
Readers, this document represents a great deal of time and effort. Enjoy. Cheers, \theauthor.
\end{preface}

% The abstract is required. Note the use of ``utabstract'' instead of
% ``abstract''! This was necessary to fix a page numbering problem.
% The abstract heading is generated automatically.
% Do NOT use \begin{abstract} ... \end{abstract}.
%
\utabstract
% \input{chapters/abstract}    % this includes the text from `abstract.tex`

\tableofcontents   % Table of Contents will be automatically
                   % generated and placed here. Required.

\listoftables      % Optional.
\listoffigures     % Optional.
\listofillustrations     % Optional.
\listofmaps      % Optional.
\listofslides    % Optional.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Actual text starts here.					     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Including external files for each chapter makes this document simpler,
% makes each chapter simpler, and allows for generating test documents
% with as few as zero chapters (by commenting out the include statements).
% Can even change the chapter order by merely interchanging the order
% of the include statements (something past contributors found helpful in their own
% dissertations =) ).
%

% \include{chapters/introduction}

% \include{chapters/main}



% NOTE: If you have only one appendix, use the command \appendix instead
% of \appendices.
%
% \appendix
\appendices

% \include{chapters/appendix}

%%%%%%%%%%%%%%%%%%%%%
% Optional glossary. May also be moved between the Table of Contents and the Text.
%%%%%%%%%%%%%%%%%%%%%
\begin{glossary}
\begin{description}
    \item[\theauthor] A hard-working graduate student, nearing the end of this chapter of your education!
    \item[\thedegree] \theauthor\ is about to earn this. Congratulations!
\end{description}
\end{glossary}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Generate the bibliography.					     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \nocite{*}    % This command causes all items in the 		     %
                % bibliographic database to be added to 	     %
                % the bibliography, even if they are not 	     %
                % explicitly cited in the text. 		     %
\bibliographystyle{plainnat}  % Here the bibliography 		     %
\bibliography{references}        % is inserted.			     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Vita page.							     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{vita}

\theauthor\ is going to graduate soon!
\end{vita}

